Spanwise wall forcing can reduce turbulent heat transfer more than drag

Direct numerical simulations are performed of turbulent forced convection in a half channel flow with wall oscillating either as a spanwise plane oscillation or to generate a streamwise travelling wave. The friction Reynolds number is fixed at $Re_{\tau_0} = 590$, but the Prandtl number $Pr$ is varied from 0.71 to 20. For $Pr>1$, the heat transfer is reduced by more than the drag, 40\% compared to 30\% at $Pr=7.5$. This outcome is related to the different responses of the velocity and thermal fields to the Stokes layer. It is shown that the Stokes layer near the wall attenuates the large-scale energy of the turbulent heat-flux and the turbulent shear-stress, but amplifies their small-scale energy. At higher Prandtl numbers, the thinning of the conductive sublayer means that the energetic scales of the turbulent heat-flux move closer to the wall, where they are exposed to a stronger Stokes layer production, increasing the contribution of the small-scale energy amplification. A predictive model is derived for the Reynolds and Prandtl number dependence of the heat-transfer reduction based on the scaling of the thermal statistics. The model agrees well with the computations for Prandtl numbers up to 20.

==> table_of_runs_reduced.tex <==
 \begin{table}
\centering
 \begin{tabular}{cc|ccc|ccc|c}
    \multicolumn{2}{c}{non-actuated} & \multicolumn{3}{c}{travelling wave} & \multicolumn{3}{c}{oscillating plane} &  \\
     \multicolumn{2}{c}{}            & \multicolumn{3}{c}{$A^+ =12, \kappa^+_x = 0.0014$} & \multicolumn{3}{c}{$A^+ =12$}         &  \\
     $L_x, L_z$ & $\Delta^+_x, \Delta^+_z$ & $\omega^+$ & $L_x, L_z$ & $\Delta^+_x, \Delta^+_z$ & $\omega^+$ & $L_x, L_z$ & $\Delta^+_x, \Delta^+_z$ & \\ \hline
%      \multicolumn{8}{c}{$Pr=0.71$} \\
            $2.7 h, 0.85 h$ & $8.3, 3.9$ &  %%% Pr = 0.71
            $0.022$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &            
            $0.022$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
     & &  
            $0.044$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &
            $0.044$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
    &  & 
            $0.066$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &
            $0.066$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & $Pr=0.71$ \\  
     & & 
            $0.088$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
            $0.088$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
     &  & 
            $0.110$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
            $0.110$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\ \\
%    \multicolumn{8}{c}{$Pr=4.0$} \\
%    full & $0.71$ & $2\pi h, \pi h$ & $8.8, 3.9$ & 
%    & &  & & & 
%    full & $0.71$ & $-0.022$ & $7.6 h, \pi h$ & $8.8, 3.9$ \\ 
%    & &  & & 
%    & &  & & & 
%    full & $0.71$ & $-0.044$ & $7.6 h, \pi h$ & $8.8, 3.9$ \\
%    & &  & & 
%    & &  & & & 
%    full  & $0.71$ & $-0.088$ & $7.6 h, \pi h$ & $8.8, 3.9$ \\   
%    \\
    $2.7 h, 0.85 h$ & $8.3, 3.9$ &   %%% Pr = 4.0     
    $0.022$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &
    $0.022$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
    &  & 
     $0.044$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &  
     $0.044$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
  &  & 
    $0.066$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &  
    $0.066$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & $Pr=4.0$ \\  
    &  & 
     $0.088$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
     $0.088$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
    &  & 
     $0.110$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &  
     $0.110$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\ \\
%      \multicolumn{8}{c}{$Pr=7.5$} \\
    $2.7 h, 0.85 h$ & $8.3, 3.9$ &  %%% Pr = 7.5 
     $0.022$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &
    $0.022$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
     &  & 
   $0.044$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
   $0.044$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
    &  & 
  $0.066$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &  
   $0.066$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & $Pr=7.5$ \\  
     &  & 
   $0.088$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
   $0.088$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
    &  & 
   $0.110$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
   $0.110$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\ \\
   $2.7 h, 0.85 h$ & $8.3, 3.9$ & 
  $0.088$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &  
     &   &   & $Pr=20.0$ \\    
%    &&&&&&&&&&&&& \\  
%  full & $7.5$ & $2\pi h, \pi h$ & $3.6, 1.8$ &  
%   full & $7.5$ & $-0.044$ & $2\pi h, \pi h$ & $3.6, 1.8$ & 
%   full  & $7.5$ & $-0.044$ & $7.6 h, \pi h$ & $3.6, 1.8$ \\
%    & &  &                                                  &
%    full  & $7.5$ & $-0.088$ & $2\pi h, \pi h$ & $3.6, 1.8$ & 
%    full  & $7.5$ & $-0.088$ & $7.6 h, \pi h$ & $3.6, 1.8$ \\  
    \end{tabular}
\caption{Production calculations at $Re_{\tau_0} = 590$   (reduced domain $L_x \ge 2.7h, L_z = 0.85h$). Non-actuated cases, see   figure~\ref{fig:flowviz_setup}(\textit{a}).  Travelling wave cases,  see figure~\ref{fig:flowviz_setup}(\textit{b}).  Spanwise plane oscillation cases, see figure~\ref{fig:flowviz_setup}(\textit{c}). }
\label{tab:runs}
\end{table}

% \caption{Summary of the production calculations for studying the effect of Prandtl number $Pr$ at different actuation frequencies $\omega^+$. The simlation cases correspond to three configurations all at $Re_\tau = 590$: non-actuated channel flow (figure~\ref{fig:flowviz_setup}\textit{a}, left side of the table), actuated channel flow with spanwise oscillating plane with $A^+ =12$ (figure~\ref{fig:flowviz_setup}\textit{c}, middle of the table), and actuated channel flow with the streamwise travelling wave with $A^+ = 12, \kappa^+_x = 0.0014$ (figure~\ref{fig:flowviz_setup}\textit{b}, right side of the table). For each configuration, we change Prandtl numbers $Pr = 0.71, 4.0, 7.5$. For the actuated cases, at each $Pr$, we perform calculations with different actuation frequencies $\omega^+$. Simulations are performed either in full domain $(L_x \ge 2\pi h, L_z = \pi h)$ or reduced domain $(L_x \ge 2.7h, L_z = 0.85h)$. The grid resolution for all cases is $\Delta^+_x \times \Delta^+_z \simeq 7.7 \times 3.9$, except for the full domain cases at $Pr = 7.5$ which have a two-times finer resolution ($\Delta^+_x \times \Delta^+_z \simeq 3.6 \times 1.8$).}


==> table_of_runs_reduced_v01.tex <==
 \begin{table}
\centering
 \begin{tabular}{ccc|ccc|ccc|c}
    \multicolumn{3}{c}{non-actuated} & \multicolumn{3}{c}{travelling wave} & \multicolumn{3}{c}{oscillating plane} &  \\
     \multicolumn{3}{c}{}            & \multicolumn{3}{c}{$A^+ =12, \kappa^+_x = 0.0014$} & \multicolumn{3}{c}{$A^+ =12$}         &  \\
     $L_x, L_z$ & $\Delta^+_x, \Delta^+_z$ & $C_{f_0}, C_{h_0}$ & $\omega^+$ & $L_x, L_z$ & $\Delta^+_x, \Delta^+_z$ & $\omega^+$ & $L_x, L_z$ & $\Delta^+_x, \Delta^+_z$ & $Pr$ \\ \hline
%      \multicolumn{8}{c}{$Pr=0.71$} \\
            $2.7 h, 0.85 h$ & $8.3, 3.9$ & $5.71 \times 10^{-3}, 3.38 \times 10^{-3}$ &  %%% Pr = 0.71
            $0.022$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &            
            $0.022$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
     & & & 
            $0.044$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &
            $0.044$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
     & & &
            $0.066$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &
            $0.066$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & $0.71$ \\  
     & & &
            $0.088$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
            $0.088$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
     & & &
            $0.110$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
            $0.110$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\ \\
%    \multicolumn{8}{c}{$Pr=4.0$} \\
%    full & $0.71$ & $2\pi h, \pi h$ & $8.8, 3.9$ & 
%    & &  & & & 
%    full & $0.71$ & $-0.022$ & $7.6 h, \pi h$ & $8.8, 3.9$ \\ 
%    & &  & & 
%    & &  & & & 
%    full & $0.71$ & $-0.044$ & $7.6 h, \pi h$ & $8.8, 3.9$ \\
%    & &  & & 
%    & &  & & & 
%    full  & $0.71$ & $-0.088$ & $7.6 h, \pi h$ & $8.8, 3.9$ \\   
%    \\
    $2.7 h, 0.85 h$ & $8.3, 3.9$ & $5.71 \times 10^{-3}, 1.41 \times 10^{-3}$ & %%% Pr = 4.0     
    $0.022$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &
    $0.022$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
    &  & &
     $0.044$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &  
     $0.044$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
  &  & &
    $0.066$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &  
    $0.066$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & $4.0$ \\  
    &  & &
     $0.088$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
     $0.088$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
    &  & &
     $0.110$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &  
     $0.110$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\ \\
%      \multicolumn{8}{c}{$Pr=7.5$} \\
    $2.7 h, 0.85 h$ & $8.3, 3.9$ & $5.71 \times 10^{-3}, 9.90 \times 10^{-4}$ &  %%% Pr = 7.5 
     $0.022$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &
    $0.022$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
     &  & &
   $0.044$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
   $0.044$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
    &  & &
  $0.066$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &  
   $0.066$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & $7.5$ \\  
     &  & &
   $0.088$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
   $0.088$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
    &  & &
   $0.110$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
   $0.110$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\ \\
   $2.7 h, 0.85 h$ & $8.3, 3.9$ & $5.71 \times 10^{-3}, 5.47 \times 10^{-4}$ & 
  $0.088$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &  
     &   &   & $Pr=20.0$ \\    
%    &&&&&&&&&&&&& \\  
%  full & $7.5$ & $2\pi h, \pi h$ & $3.6, 1.8$ &  
%   full & $7.5$ & $-0.044$ & $2\pi h, \pi h$ & $3.6, 1.8$ & 
%   full  & $7.5$ & $-0.044$ & $7.6 h, \pi h$ & $3.6, 1.8$ \\
%    & &  &                                                  &
%    full  & $7.5$ & $-0.088$ & $2\pi h, \pi h$ & $3.6, 1.8$ & 
%    full  & $7.5$ & $-0.088$ & $7.6 h, \pi h$ & $3.6, 1.8$ \\  
    \end{tabular}
\caption{Production calculations at $Re_{\tau_0} = 590$   (reduced domain $L_x \ge 2.7h, L_z = 0.85h$). Non-actuated cases, see   figure~\ref{fig:flowviz_setup}(\textit{a}).  Travelling wave cases,  see figure~\ref{fig:flowviz_setup}(\textit{b}).  Spanwise plane oscillation cases, see figure~\ref{fig:flowviz_setup}(\textit{c}). }
\label{tab:runs}
\end{table}

% \caption{Summary of the production calculations for studying the effect of Prandtl number $Pr$ at different actuation frequencies $\omega^+$. The simlation cases correspond to three configurations all at $Re_\tau = 590$: non-actuated channel flow (figure~\ref{fig:flowviz_setup}\textit{a}, left side of the table), actuated channel flow with spanwise oscillating plane with $A^+ =12$ (figure~\ref{fig:flowviz_setup}\textit{c}, middle of the table), and actuated channel flow with the streamwise travelling wave with $A^+ = 12, \kappa^+_x = 0.0014$ (figure~\ref{fig:flowviz_setup}\textit{b}, right side of the table). For each configuration, we change Prandtl numbers $Pr = 0.71, 4.0, 7.5$. For the actuated cases, at each $Pr$, we perform calculations with different actuation frequencies $\omega^+$. Simulations are performed either in full domain $(L_x \ge 2\pi h, L_z = \pi h)$ or reduced domain $(L_x \ge 2.7h, L_z = 0.85h)$. The grid resolution for all cases is $\Delta^+_x \times \Delta^+_z \simeq 7.7 \times 3.9$, except for the full domain cases at $Pr = 7.5$ which have a two-times finer resolution ($\Delta^+_x \times \Delta^+_z \simeq 3.6 \times 1.8$).}


==> table_of_runs_reduced_v02.tex <==
 \begin{table}
\centering
 \begin{tabular}{cc|ccc|ccc|c}
    \multicolumn{2}{c|}{non-actuated} & \multicolumn{3}{c|}{travelling wave} & \multicolumn{3}{c|}{oscillating plane} &  \\
     \multicolumn{2}{c|}{}            & \multicolumn{3}{c|}{$A^+ =12, \kappa^+_x = 0.0014$} & \multicolumn{3}{c|}{$A^+ =12$}         &  \\
     \multicolumn{2}{c|}{$L_x \times L_z = 2.7 h \times 0.85 h$}            & \multicolumn{3}{c|}{$L_x \times L_z = 7.6 h \times 0.85 h$} & \multicolumn{3}{c|}{$L_x \times L_z = 2.7 h \times 0.85 h$}         &  \\ 
     \multicolumn{2}{c|}{}            & \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{}         &  \\
     $\Delta^+_x, \Delta^+_z$ & $\Delta^+_{y_w}, \Delta^+_{y_c}$ & $\omega^+$ & $\Delta^+_x, \Delta^+_z$ & $\Delta^+_x, \Delta^+_z$ & $\omega^+$ & $\Delta^+_x, \Delta^+_z$ & $\Delta^+_x, \Delta^+_z$ & \\ \hline
%      \multicolumn{8}{c}{$Pr=0.71$} \\
            $8.3, 3.9$ & $0.3, 8.5$ &  %%% Pr = 0.71
            $0.022$ & $8.8, 3.9$ & $8.8, 3.9$ &            
            $0.022$ & $8.3, 3.9$ & $8.3, 3.9$ & \\
     & &  
            $0.044$ & $8.8, 3.9$ & $8.8, 3.9$ &
            $0.044$ & $8.3, 3.9$ & $8.3, 3.9$ & \\
    &  & 
            $0.066$ & $8.8, 3.9$ & $8.8, 3.9$ &
            $0.066$ & $8.3, 3.9$ & $8.3, 3.9$ & $Pr=0.71$ \\  
     & & 
            $0.088$ & $8.8, 3.9$ & $8.8, 3.9$ & 
            $0.088$ & $8.3, 3.9$ & $8.3, 3.9$ & \\
     &  & 
            $0.110$ & $8.8, 3.9$ & $8.8, 3.9$ & 
            $0.110$ & $8.3, 3.9$ & $8.3, 3.9$ & \\ \\
%    \multicolumn{8}{c}{$Pr=4.0$} \\
%    full & $0.71$ & $2\pi h, \pi h$ & $8.8, 3.9$ & 
%    & &  & & & 
%    full & $0.71$ & $-0.022$ & $7.6 h, \pi h$ & $8.8, 3.9$ \\ 
%    & &  & & 
%    & &  & & & 
%    full & $0.71$ & $-0.044$ & $7.6 h, \pi h$ & $8.8, 3.9$ \\
%    & &  & & 
%    & &  & & & 
%    full  & $0.71$ & $-0.088$ & $7.6 h, \pi h$ & $8.8, 3.9$ \\   
%    \\
    $8.3, 3.9$ & $0.3, 8.5$ &   %%% Pr = 4.0     
    $0.022$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &
    $0.022$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
    &  & 
     $0.044$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &  
     $0.044$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
  &  & 
    $0.066$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &  
    $0.066$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & $Pr=4.0$ \\  
    &  & 
     $0.088$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
     $0.088$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
    &  & 
     $0.110$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &  
     $0.110$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\ \\
%      \multicolumn{8}{c}{$Pr=7.5$} \\
    $8.3, 3.9$ & $0.3, 8.5$ &  %%% Pr = 7.5 
     $0.022$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &
    $0.022$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
     &  & 
   $0.044$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
   $0.044$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
    &  & 
  $0.066$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &  
   $0.066$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & $Pr=7.5$ \\  
     &  & 
   $0.088$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
   $0.088$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\
    &  & 
   $0.110$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & 
   $0.110$ & $2.7 h, 0.85 h$ & $8.3, 3.9$ & \\ \\
   $8.3, 3.9$ & $0.3, 8.4$ & 
  $0.088$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ &  
     &   &   & $Pr=20.0$ \\    
%    &&&&&&&&&&&&& \\  
%  full & $7.5$ & $2\pi h, \pi h$ & $3.6, 1.8$ &  
%   full & $7.5$ & $-0.044$ & $2\pi h, \pi h$ & $3.6, 1.8$ & 
%   full  & $7.5$ & $-0.044$ & $7.6 h, \pi h$ & $3.6, 1.8$ \\
%    & &  &                                                  &
%    full  & $7.5$ & $-0.088$ & $2\pi h, \pi h$ & $3.6, 1.8$ & 
%    full  & $7.5$ & $-0.088$ & $7.6 h, \pi h$ & $3.6, 1.8$ \\  
    \end{tabular}
\caption{Production calculations at $Re_{\tau_0} = 590$   (reduced domain $L_x \ge 2.7h, L_z = 0.85h$). Non-actuated cases, see   figure~\ref{fig:flowviz_setup}(\textit{a}).  Travelling wave cases,  see figure~\ref{fig:flowviz_setup}(\textit{b}).  Spanwise plane oscillation cases, see figure~\ref{fig:flowviz_setup}(\textit{c}). }
\label{tab:runs}
\end{table}

% \caption{Summary of the production calculations for studying the effect of Prandtl number $Pr$ at different actuation frequencies $\omega^+$. The simlation cases correspond to three configurations all at $Re_\tau = 590$: non-actuated channel flow (figure~\ref{fig:flowviz_setup}\textit{a}, left side of the table), actuated channel flow with spanwise oscillating plane with $A^+ =12$ (figure~\ref{fig:flowviz_setup}\textit{c}, middle of the table), and actuated channel flow with the streamwise travelling wave with $A^+ = 12, \kappa^+_x = 0.0014$ (figure~\ref{fig:flowviz_setup}\textit{b}, right side of the table). For each configuration, we change Prandtl numbers $Pr = 0.71, 4.0, 7.5$. For the actuated cases, at each $Pr$, we perform calculations with different actuation frequencies $\omega^+$. Simulations are performed either in full domain $(L_x \ge 2\pi h, L_z = \pi h)$ or reduced domain $(L_x \ge 2.7h, L_z = 0.85h)$. The grid resolution for all cases is $\Delta^+_x \times \Delta^+_z \simeq 7.7 \times 3.9$, except for the full domain cases at $Pr = 7.5$ which have a two-times finer resolution ($\Delta^+_x \times \Delta^+_z \simeq 3.6 \times 1.8$).}


==> table_of_runs_support.tex <==
 \begin{table}
\centering
 \begin{tabular}{cc|ccc|ccc|c}
    \multicolumn{2}{c}{non-actuated} & \multicolumn{3}{c}{oscillating plane} & \multicolumn{3}{c}{travelling wave} &  \\
     \multicolumn{2}{c}{}            & \multicolumn{3}{c}{$A^+ =12$}         & \multicolumn{3}{c}{$A^+ =12, \kappa^+_x = 0.0014$} &  \\
     $L_x, L_z$ & $\Delta^+_x, \Delta^+_z$ & $\omega^+$ & $L_x, L_z$ & $\Delta^+_x, \Delta^+_z$ & $\omega^+$ & $L_x, L_z$ & $\Delta^+_x, \Delta^+_z$ &  \\  \hline
%      \multicolumn{8}{c}{$Pr=0.71$} & \\
            $2\pi h, \pi h$ & $7.7, 3.9$ &  %%% Pr = 0.71
            & & &
            $-0.022$ & $7.6 h, \pi h$ & $7.4, 3.9$ &  \\
            & & 
            & & &
            $-0.044$ & $7.6 h, \pi h$ & $7.4, 3.9$ & $Pr=0.71$ \\  
            & & 
            & & &
            $-0.088$ & $7.6 h, \pi h$ & $7.4, 3.9$ &   \\ \\
%      \multicolumn{8}{c}{$Pr=7.5$} \\
    $2\pi h, \pi h$ & $3.6, 1.8$ &  %%% Pr = 7.5
    $-0.044$ & $2\pi h, \pi h$ & $3.6, 1.8$ & 
    $-0.044$ & $7.6 h, \pi h$ & $3.9, 1.8$ & \\
      &   &  %%% Pr = 7.5
      &   &   & 
    $-0.044$ & $7.6 h, \pi h$ & $5.8, 2.7$ & \\
      &   &  %%% Pr = 7.5
      &   &  & 
    $-0.044$ & $7.6 h, \pi h$ & $8.8, 4.0$ & $Pr=7.5$ \\    
     &  & 
   $-0.088$ & $2\pi h, \pi h$ & $3.6, 1.8$ & 
   $-0.088$ & $7.6 h, \pi h$ & $3.9, 1.8$ & \\ \\ 
%      \multicolumn{8}{c}{$Pr=20.0$} \\
    $2.7 h, 0.85 h$ & $8.3, 3.9$ &  %%% Pr = 7.5
      &   &   & 
    $-0.088$ & $7.6 h, 0.85 h$ & $8.8, 3.9$ & \\
    $2.7 h, 0.85 h$ & $6.2, 2.6$ & 
     &   &   & 
    $-0.088$ & $7.6 h, 0.85 h$ & $5.8, 3.9$ & $Pr=20.0$ \\ 
    $2.7 h, 0.85 h$ & $4.1, 2.0$ & 
     &   &   & 
    $-0.088$ & $7.6 h, 0.85 h$ & $4.4, 2.0$ & \\    
    \end{tabular}
\caption{Summary of the additional calculations for validation study at $Re_\tau = 590$. The cases at $Pr=0.71$ (top three rows) and $Pr=7.5$ (middle four rows) are for validating the domain and the grid size for the production runs in table~\ref{tab:runs}. The results of the validation are reported in Appendix~\ref{sec:grid_domain} and figure~\ref{fig:averaged_HR_DR_Pr}. The cases at $Pr=20.0$ are for evaluating the prediction model for $HR$ (\S\ \ref{sec:hr_model}).
}
\label{tab:runs_support}
\end{table}

% \caption{Summary of the production calculations for studying the effect of Prandtl number $Pr$ at different actuation frequencies $\omega^+$. The simlation cases correspond to three configurations all at $Re_\tau = 590$: non-actuated channel flow (figure~\ref{fig:flowviz_setup}\textit{a}, left side of the table), actuated channel flow with spanwise oscillating plane with $A^+ =12$ (figure~\ref{fig:flowviz_setup}\textit{c}, middle of the table), and actuated channel flow with the streamwise travelling wave with $A^+ = 12, \kappa^+_x = 0.0014$ (figure~\ref{fig:flowviz_setup}\textit{b}, right side of the table). For each configuration, we change Prandtl numbers $Pr = 0.71, 4.0, 7.5$. For the actuated cases, at each $Pr$, we perform calculations with different actuation frequencies $\omega^+$. Simulations are performed either in full domain $(L_x \ge 2\pi h, L_z = \pi h)$ or reduced domain $(L_x \ge 2.7h, L_z = 0.85h)$. The grid resolution for all cases is $\Delta^+_x \times \Delta^+_z \simeq 7.7 \times 3.9$, except for the full domain cases at $Pr = 7.5$ which have a two-times finer resolution ($\Delta^+_x \times \Delta^+_z \simeq 3.6 \times 1.8$).}

